SoK: A Taxonomy for Distributed-Ledger-Based Identity Management

The intersection of blockchain (distributed ledger) and identity management lacks a comprehensive framework for classifying distributed-ledger-based identity solutions. This paper introduces a methodologically developed taxonomy derived from the analysis of 390 scientific papers and expert discussions. The resulting framework consists of 22 dimensions with 113 characteristics, organized into three groups: trust anchor implementations, identity architectures (identifiers and credentials), and ledger specifications. This taxonomy facilitates the systematic analysis, comparison, and design of distributed-ledger-based identity solutions, as demonstrated through its application to two distinct architectures. As the first methodology-driven taxonomy in this field, this work advances standardization and enhances understanding of distributed-ledger-based identity architectures. It provides researchers and practitioners with a structured framework for evaluating design decisions and implementation approaches.

==> archive/5_Evaluation.tex <==
\section{Evaluation}
\label{sec:evaluation}
% Goals copied from section 3:
% \item Provide a Detailed and Holistic Overview: By offering a comprehensive report on blockchain-based IDM architectures, we aim to surpass other taxonomies in this area that only provide specific excerpts.
% \item Enhance Understanding and Comparability: Facilitate a deeper understanding of the phenomenon and make solutions conceptually comparable by identifying and utilizing the fundamental building blocks and components of blockchain-based IDM solutions.
This section evaluates the developed taxonomy based on predefined criteria. The objective ending conditions were met, as stated in the previous section. Next, the subjective ending conditions are checked, as listed in \autoref{tab:ending-conditions}. The subjective ending conditions S2-S5 (Robustness, Comprehensiveness, Extendibility, and Explanatory Power) are met. We tested with domain experts and practitioners that the taxonomy meaningful differentiates between objects, covers all relevant dimensions, is extendable, and provides insights and explanations for understanding the domain. Ending condition, S1 (Conciseness), meaning the taxonomy is simple and practical, is partially met due to its relative length of \numberdimensions\ dimensions and \numbercharacteristics\ characteristics. However, presenting a comprehensive taxonomy was a deliberate decision aligned with our evaluation goals. These goals aim to provide a detailed and holistic overview while enhancing understanding and facilitating communication. 

We consider the evaluation goals to be achieved for several reasons. First, we followed a structured approach grounded in the most extensive body of literature available for this type of taxonomy in our research area. Second, every dimension of the taxonomy underwent multiple revisions, reviews, and tests with domain and industry experts. Third, we successfully tested our taxonomy artifact against existing taxonomies and meta-analyses in this field. Overall, these rigorous processes ensure that our taxonomy is both robust and comprehensive, meeting the intended objectives.



==> archive/table_taxonomy_Awid1.tex <==
   % Define the macro
   \newcommand{\GrayDimension}[9]{%
       % Dimension Grey
       \rowcolor{gray!10} 
       \cellcolor{white} &
       & \rule{0pt}{2ex}#2
       & #3 	
       & #4 
       & #5 \\ 
       \cline{3-6} 
       \rowcolor{gray!10}
       \cellcolor{white} &
       \rule{0pt}{2ex}\multirow{-2}{0.15\textwidth}{\cellcolor{gray!10}\centering 
       #1} 
       & \rule{0pt}{2ex}#6& #7& #8&#9 \\ 
       \Xcline{2-6}{0.8pt}
   }
      \newcommand{\WhiteDimension}[9]{%
       % Dimension White
        & \rule{0pt}{2ex}\multirow{-0.9}{0.15\textwidth}{\centering #1} & #2 & #3 & #4 & #5 \\ \cline{3-6}
                                     & & \rule{0pt}{2ex}#6 & #7 & #8 & #9 \\ 
        % HELP ME HERE WITH DRAWING A LINE I TRIED MANY SOLUTIONS BUT NOTHING WORKS 
        % \arrayrulecolor{black}\Xcline{2-6}{0.8pt}\arrayrulecolor{black}
        % \hhline{>{\arrayrulecolor{black}}|~|>{\arrayrulecolor{black}}-----}
        % \arrayrulecolor{black}\Xcline{2-6}{0.8pt}
        % \hline\noalign{\hrule height 0.6pt}
        
   }

\begin{table*}
    \centering
    \renewcommand{\arraystretch}{1}
    \arrayrulecolor{black}
    % \begin{tabular}{!{\vrule width 1pt}p{0.15\textwidth}!{\vrule width 0.6pt}p{0.18\textwidth}|p{0.18\textwidth}|p{0.18\textwidth}|p{0.18\textwidth}!{\vrule width 1pt}}

   \begin{tabular}{!{\vrule width 1pt}p{0.02\textwidth}!{\vrule width 1pt}p{0.15\textwidth}!{\vrule width 0.6pt}p{0.18\textwidth}|p{0.18\textwidth}|p{0.18\textwidth}|p{0.18\textwidth}!{\vrule width 1pt}}
    
    \hline\noalign{\hrule height 1pt}
    
    % \rule{0pt}{3ex}\centering\textbf{Dimension} & \multicolumn{4}{c!{\vrule width 1pt}}{\textbf{Characteristics}} \rule[-1.5ex]{0pt}{0pt}\\ 
    % \hline\noalign{\hrule height 1.1pt}

    \rule{0pt}{3ex} & \centering\textbf{Dimension} & \multicolumn{4}{c!{\vrule width 1pt}}{\textbf{Characteristics}} \rule[-1.5ex]{0pt}{0pt}\\
    \noalign{\hrule height 1.1pt}
    
%% Group 1: Architectural, Technical Infrastructure, and Governance Aspects

    %Dimension Grey
    % Identity Management Architecture
    \GrayDimension{Identity Management Architecture}{Centralized}{Federated}{Decentralized}{Self-Sovereign}{}{}{}{}
        
    %Dimension White Governance Structure
    \WhiteDimension{Governance Structure}{Centralized}{Consortium}{Decentralized}{Autonomous}{Hybrid}{}{}{}

%     %Dimension Grey \GrayDimension{}{}{}{}{}{}{}{}{}
 % Central Authority & Trusted Third Parties & Trust Registries / Lists & Hardware-Based \\ 
    \GrayDimension{Trust Anchor Implementation}{Central Authority}{Trusted Third Parties}{Trust Registries / Lists}{Hardware-Based}{Decentralized PKI}{Web of Trust}{}{}
            
%     %Dimension White
%     \rule{0pt}{2ex}\multirow{-0.9}{0.15\textwidth}{\centering Consensus Mechanism } & Proof-of-Work&Proof-of-Stake &Proof-of-Authority &Delegated Proof-of-Stake \\ \cline{2-5}
%                                  & \rule{0pt}{2ex}Byzantine Fault Tolerance &Other Consensus Mechanisms & &\\ 
%     \hline\noalign{\hrule height 0.6pt}

%     %Dimension Grey \GrayDimension{}{}{}{}{}{}{}{}{}
%     \rowcolor{gray!10}
%     \rule{0pt}{2ex}\multirow{-0.9}{0.15\textwidth}{\cellcolor{gray!10}\centering Ledger Type} & Public Permissionless & Public Permissioned & Private Permissioned & Consortium \\ \cline{2-5}
%     \rowcolor{gray!10}
%     \rule{0pt}{2ex} & Hybrid & Other & & \\
%     \hline\noalign{\hrule height 0.6pt}

%     %Dimension White
%     \rule{0pt}{2ex}\multirow{-0.9}{0.15\textwidth}{\centering Identity Data Storage Location} & On-Chain Storage & Off-Chain Central. Storage & Off-Chain Decentral. Storage & Local User Storage \\ \cline{2-5}
%     \rule{0pt}{2ex} & Hybrid Storage & No Data Stored & & \\
%     \hline\noalign{\hrule height 0.6pt}

%     %Dimension Grey
%     \rowcolor{gray!10}
%     \rule{0pt}{2ex}& No On-Chain Data & Hashed Data On-Chain & Encrypted Data On-Chain & Plain Text Data On-Chain \\ \cline{2-5}
%     \rowcolor{gray!10}
%     \rule{0pt}{2ex}\multirow{-2}{0.15\textwidth}{\cellcolor{gray!10}\centering On-Chain Data Visibility} & \rule{0pt}{2ex} &  &  &  \\ 
%     \hline\noalign{\hrule height 0.6pt}

%     %Dimension White
%     \rule{0pt}{2ex}\multirow{-0.9}{0.15\textwidth}{\centering Credential Storage Location} & On-Chain & Off-Chain Centralized  & Off-Chain Decentralized & Hybrid Storage \\ \cline{2-5}
%     \rule{0pt}{2ex} & Mirrored Storage & & & \\
%     \hline\noalign{\hrule height 0.6pt}

%     %Dimension Grey
%     \rowcolor{gray!10}
%     \rule{0pt}{2ex}&Open Source & Closed Source &  &  \\ \cline{2-5}
%     \rowcolor{gray!10}
%     \rule{0pt}{2ex}\multirow{-2}{0.15\textwidth}{\cellcolor{gray!10}\centering Technical Transparency} & \rule{0pt}{2ex} &  &  &  \\ 
%     \hline\noalign{\hrule height 0.6pt}

%     %Dimension White
%     \rule{0pt}{2ex}\multirow{-0.9}{0.15\textwidth}{\centering Cost Model (Excluding Blockchain Fees)} & No Fees & Creation Fee Only & Usage Fee Only & Creation and Usage Fees \\ \cline{2-5}
%     \rule{0pt}{2ex} & Token-Based Fee Model & Alternative Fee Models & & \\
%     \hline\noalign{\hrule height 0.6pt}
    
%    %Dimension White
%        \rowcolor{gray!10}
%     \rule{0pt}{2ex}& Identity Tokenization & Validation Mechanisms & Credential Anchoring & Credential Storage \\ \cline{2-5}
%     \rowcolor{gray!10}
%     \rule{0pt}{2ex}\multirow{-2}{0.17\textwidth}{\cellcolor{gray!10}\centering Blockchain Functionality for Identity} & \rule{0pt}{2ex}  DID resolving & Smart Contract Processes & Access Control & \\ 
%     \hline\noalign{\hrule height 0.8pt}



    
    

% %% Group 2: Identity and Credential Lifecycle and User Experience

%     %Dimension White
%     \rule{0pt}{2ex}\multirow{-0.9}{0.15\textwidth}{\centering Identity Subject Type} & Human Individuals & Organizations & Devices & Software Applications \\ \cline{2-5}
%                                  & \rule{0pt}{2ex}Smart Contracts & Digital Assets & Autonomous Agents & Processes/Services \\ 
%     \hline\noalign{\hrule height 0.6pt}

%     %Dimension Grey
%     \rowcolor{gray!10}
%     \rule{0pt}{2ex}\multirow{-0.9}{0.15\textwidth}{\cellcolor{gray!10}\centering Credential Binding Method to Subject} & Public Key Association & Transferable Tokens & Non-Transferable Tokens & Soulbound Tokens \\ \cline{2-5}
%     \rowcolor{gray!10}
%     \rule{0pt}{2ex} & Registry-Based Association & Anonymous Credentials & & \\
%     \hline\noalign{\hrule height 0.6pt}

%     %Dimension White
%     \rule{0pt}{2ex}\multirow{-0.9}{0.15\textwidth}{\centering Identity Representation Mechanism} & NFT-Based & Digital Identity Certificates & Public Key-Based & Identity Registries \\ \cline{2-5}
%     & \rule{0pt}{2ex} Soulbound Tokens & Verifiable Credentials & No Explicit Representation & \\ 
%     \hline\noalign{\hrule height 0.6pt}

%     %Dimension Grey
%     \rowcolor{gray!10}
%     \rule{0pt}{2ex}\multirow{-0.9}{0.15\textwidth}{\cellcolor{gray!10}\centering Credential Issuance Model} & Self-Issued Credentials & Single External Issuer & Multiple Collaborative Issuers & Multiple Independent Issuers \\ \cline{2-5}
%     \rowcolor{gray!10}
%     \rule{0pt}{2ex} & Hybrid Issuance Model & & & \\
%     \hline\noalign{\hrule height 0.6pt}

%     %Dimension White
%     \rule{0pt}{2ex}\multirow{-0.9}{0.15\textwidth}{\centering Credential Lifespan} & Permanent Credentials & Time-Limited Credentials & Activity-Based Credentials & Ephemeral Credentials \\ \cline{2-5}
%     & \rule{0pt}{2ex} & &  & \\ 
%     \hline\noalign{\hrule height 0.6pt}

%     %Dimension Grey
%     \rowcolor{gray!10}
%     \rule{0pt}{2ex}&Fully Transferable & Non-Transferable & Conditionally Transferable & Delegable Rights  \\ \cline{2-5}
%     \rowcolor{gray!10}
%     \rule{0pt}{2ex}\multirow{-2}{0.15\textwidth}{\cellcolor{gray!10}\centering Credential Transferability} & \rule{0pt}{2ex} &  &  &  \\ 
%     \hline\noalign{\hrule height 0.6pt}
        
%     %Dimension White
%     \rule{0pt}{2ex}\multirow{-0.9}{0.15\textwidth}{\centering Recovery Mechanisms} & Social Recovery & Institutional Recovery & Biometric Recovery & No Recovery Mechanism \\ \cline{2-5}
%     \rule{0pt}{2ex} & Other Recovery Mechanism & & & \\
%     \hline\noalign{\hrule height 0.6pt}

%     %Dimension Grey
%     \rowcolor{gray!10}
%     \rule{0pt}{2ex}& Universal Claim Addition &	Restricted Claim Addition  &  &  \\ \cline{2-5}
%     \rowcolor{gray!10}
%     \rule{0pt}{2ex}\multirow{-2}{0.15\textwidth}{\cellcolor{gray!10}\centering Claim Addition Rights} & \rule{0pt}{2ex} &  &  &  \\ 
%     \hline\noalign{\hrule height 0.6pt}

%     %Dimension White
%     \rule{0pt}{2ex}\multirow{-0.9}{0.15\textwidth}{\centering Identifier Type} & Logical Identifiers & Physical Identifiers & & \\ \cline{2-5}
%                                  & \rule{0pt}{2ex} & &  & \\ 
%     \hline\noalign{\hrule height 0.6pt}

%     %Dimension Grey
%     \rowcolor{gray!10}
%     \rule{0pt}{2ex}& Subject-Provided Claims & Third-Party Claims & Combined Claims & \\ \cline{2-5}
%     \rowcolor{gray!10}
%     \rule{0pt}{2ex}\multirow{-2}{0.15\textwidth}{\cellcolor{gray!10}\centering Initial Claim Provider} & \rule{0pt}{2ex} &  &  &  \\ 
%     \hline\noalign{\hrule height 0.6pt}

%     %Dimension White
%     \rule{0pt}{2ex}\multirow{-0.9}{0.15\textwidth}{\centering Privacy Level} & Anonymous Identity & Pseudonymous Identity & Linked Real Identity & \\ \cline{2-5}
%     & \rule{0pt}{2ex} & &  & \\ 
%         \hline\noalign{\hrule height 0.6pt}

%     %Dimension Grey
%     \rowcolor{gray!10}
%     \rule{0pt}{2ex}\multirow{-0.9}{0.15\textwidth}{\cellcolor{gray!10}\centering Authentication Mechanism} & Password-Based & Private Key & Hardware Token & Third-Party \\ \cline{2-5}
%     \rowcolor{gray!10}
%     \rule{0pt}{2ex} & Delegated  & One-Time Passwords (OTP) & Biometric  & Multi-Factor (MFA) \\
%     \hline\noalign{\hrule height 0.6pt}

    %     %Dimension White
    % \rule{0pt}{2ex}\multirow{-0.9}{0.15\textwidth}{\centering Credential Verifiability} & Non-Verifiable Credentials & Verifiable with Issuer Interaction & Verifiable without Issuer Interaction & \\ 
    % \hline\noalign{\hrule height 0.6pt}
    
    % Example
    % %Dimension Grey
    % \rowcolor{gray!10}
    % \rule{0pt}{2ex}& &  &  &  \\ \cline{2-5}
    % \rowcolor{gray!10}
    % \rule{0pt}{2ex}\multirow{-2}{0.15\textwidth}{\cellcolor{gray!10}\centering } & \rule{0pt}{2ex} &  &  &  \\ 
    % \hline\noalign{\hrule height 0.6pt}
        
    % %Dimension White
    % \rule{0pt}{2ex}\multirow{-0.9}{0.15\textwidth}{\centering } & & & & \\ \cline{2-5}
    % & \rule{0pt}{2ex} & &  & \\ 
    % \hline\noalign{\hrule height 0.6pt}
    
    %End Table
    \end{tabular}
    \vspace{0.5em}
    \caption{Table caption describing the taxonomy dimensions and their characteristics}
    \label{tab:taxonomy-v1}
\end{table*}

    






==> archive/table_taxonomy_dimensions_and_char.tex <==
% Include the following packages in your preamble:
% \usepackage{rotating}
% \usepackage{booktabs}
% \usepackage{tabularx}
% \usepackage{array}

% Table code:

\begin{table}
\centering
\small % Increase font size
\caption{Dimensions and Characteristics of Blockchain-based Identity Systems}
\label{tab:dimensions}
\begin{tabularx}{\textwidth}{>{\hsize=0.25\hsize}X >{\hsize=0.75\hsize}X}
\toprule
\textbf{Dimension} & \textbf{Characteristics} \\
\midrule
% Dimension 1
\textbf{1. Identity Data Storage Location} &
On-Chain Storage; Off-Chain Storage with On-Chain References; Off-Chain Storage Without On-Chain References; Hybrid Storage \\
\midrule
% Dimension 2
\textbf{2. Identity Verification Method} &
On-Chain Verification; Off-Chain Verification; Hybrid Verification \\
\midrule
% Dimension 3
\textbf{3. Identity Usage Context} &
On-Chain Usage; Off-Chain Usage; Both On-Chain and Off-Chain Usage \\
\midrule
% Dimension 4
\textbf{4. Identity Data Granularity} &
Full Identity Data; Partial Identity Data; Minimal Disclosure (Zero-Knowledge Proofs) \\
\midrule
% Dimension 5
\textbf{5. Identity Data Control} &
User-Controlled Identity; Third-Party Controlled Identity; Shared Control \\
\midrule
% Dimension 6
\textbf{6. Privacy Level} &
Public Identity Data; Private/Encrypted Identity Data; Anonymous Credentials \\
\midrule
% Dimension 7
\textbf{7. Trust Model} &
Self-Sovereign Identity; Federated Identity; Centralized Identity \\
\midrule
% Dimension 8
\textbf{8. Identity Lifecycle Management} &
Supports Revocation; Does Not Support Revocation; Supports Updates; Immutable Identity Data \\
\midrule
% Dimension 9
\textbf{9. User Anonymity} &
Anonymous; Pseudonymous; Identified \\
\midrule
% Dimension 10
\textbf{10. Data Storage Mechanism} &
Blockchain Storage; Distributed File Systems (e.g., IPFS); Centralized Databases; Cloud Storage \\
\midrule
% Dimension 11
\textbf{11. Type of Blockchain} &
Public Blockchain; Private Blockchain; Consortium Blockchain; Permissioned Blockchain \\
\midrule
% Dimension 12
\textbf{12. Credential Type} &
Verifiable Credentials; Decentralized Identifiers (DIDs); Traditional Credentials; Biometric Credentials \\
\midrule
% Dimension 13
\textbf{13. Authentication Mechanism} &
Password-Based Authentication; Cryptographic Keys; Biometric Authentication; Multi-Factor Authentication (MFA) \\
\midrule
% Dimension 14
\textbf{14. Smart Contract Utilization} &
Uses Smart Contracts; Does Not Use Smart Contracts; Limited Use of Smart Contracts \\
\midrule
% Dimension 15
\textbf{15. Interoperability} &
Interoperable with Other Blockchain Systems; Interoperable with Traditional Systems; Standalone System \\
\midrule
% Dimension 16
\textbf{16. Compliance with Regulations} &
GDPR Compliant; Non-Compliant; Region-Specific Compliance; Compliance Agnostic \\
\midrule
% Dimension 17
\textbf{17. Identity Data Immutability} &
Immutable Data; Mutable Data; Versioned Data \\
\midrule
% Dimension 18
\textbf{18. Scalability} &
High Scalability; Limited Scalability; Scalability Through Layer 2 Solutions \\
\midrule
% Dimension 19
\textbf{19. Security Measures} &
Standard Cryptography; Advanced Cryptography (e.g., Quantum-Resistant); Multi-Factor Authentication; Hardware Security Modules (HSMs) \\
\midrule
% Dimension 20
\textbf{20. Cost Model} &
Transaction Fees Required; Free Transactions; Subscription-Based; Freemium Model \\
\bottomrule
\end{tabularx}
\end{table}


==> archive/table_taxonomy_v1_Sandro.tex <==

\begin{table*}
    \begin{tblr}{
        % Column specifications with relative widths and alignment
        colspec = {|[1.5pt] X[0.08,c]|[1.5pt] X[0.25,c]|X[0.7,c]| [1.5pt] X[c]},
        % Basic table structure
        hlines, vlines,
        % Column spacing adjustments
        column{3-3}={colsep=20pt}, 
        column{2-2}={colsep=10pt}, 
        % Row styling
        rows = {m},                % Middle vertical alignment
        row{1} = {font=\bfseries}, % Bold header
        rowsep = 1.5pt,           % Default row separation
        row{1} = {rowsep=4pt},
        row{2-24} = {rowsep=2pt}, % Consistent row height for content
        % Explicit alternating backgrounds
        row{2-2} = {bg=gray!10},
        row{4-4} = {bg=gray!10},
        row{6-6} = {bg=gray!10},
        row{8-8} = {bg=gray!10},
        row{10-10} = {bg=gray!10},
        row{12-12} = {bg=gray!10},
        row{14-14} = {bg=gray!10},
        row{16-16} = {bg=gray!10},
        row{18-18} = {bg=gray!10},
        row{20-20} = {bg=gray!10},
        row{22-22} = {bg=gray!10},
        row{24-24} = {bg=gray!10},
        % Major section dividers (thicker lines)
        hline{1} = {1-6}{1.5pt},   % Top border
        hline{2} = {1-6}{1.5pt},   % Below header
        hline{10} = {1-6}{1.5pt},  % After Group 1
        hline{13} = {1-6}{1.5pt},  % After Group 2
        hline{25} = {1-6}{1.5pt},  % Bottom border
        % Subsection dividers (thinner lines)
        hline{4,6,8,12,14,16,20,22} = {2-6}{0.9pt}
    }
    % Header Row
    \SetCell[c=1]{c}\textbf{Group} &
    \SetCell[c=1]{c}\textbf{Dimension} &
    \SetCell[c=1]{c}\textbf{Characteristics} \\

    % GROUP 1: Technical Architecture and Governance
    \SetCell[r=8]{c,bg=white}{\rotatebox{90}{\parbox{4cm}{\centering \small \textbf{Technical Architecture and Governance}}}} &
    % Identity Management Architecture
    \SetCell[r=1]{c}{\textbf{Identity Management Architecture}} &
     Decentralized \textbullet\  Centralized \textbullet\  Federated \textbullet\  Poly-Centric \textbullet\ Self-Sovereign \textbullet\ Siloed \textbullet\ Hybrid \\
  
    % System Governance Structure
    &
    \SetCell[r=1]{c}{\textbf{System Governance Structure}} &
    Centralized \textbullet\ Consortium \textbullet\ Decentralized \textbullet\ Autonomous \textbullet\
    Hybrid \\
  
    % Trust Anchor Implementation
    &
    \SetCell[r=1]{c}{\textbf{Trust Anchor Implementation}} &
    Central Authority \textbullet\ Trusted Third Parties \textbullet\ Decentral. Trust Registries \textbullet\ Hardware-Based \textbullet\ Decentralized PKI \textbullet\ Web of Trust \\
  
    % Identifier Location
    &
    \SetCell[r=1]{c}{\textbf{Identifier Location}} &
    On-Chain Storage \textbullet\ Off-Chain Central. Storage \textbullet\ Off-Chain Decentr. Storage \textbullet\ Local User Storage \textbullet\ Hybrid Storage \textbullet\ No Data Stored \\
  
    % On-Chain Data Visibility
    &
    \SetCell[r=1]{c}{\textbf{On-Chain Data Visibility}} &
    No On-Chain Data \textbullet\ Hashed Data On-Chain \textbullet\ Encrypted Data On-Chain \textbullet\ Plain Text Data On-Chain \\
  
    % Credential Storage Location
    &
    \SetCell[r=1]{c}{\textbf{Credential Storage Location}} &
    On-Chain \textbullet\ Off-Chain Centralized \textbullet\ Off-Chain Decentralized \textbullet\ Off-Chain at Subject \textbullet\ On\&Off-Chain Hybrid \textbullet\ On\&Off-Chain Decentral. \\
  
    % Cost Model
    &
    \SetCell[r=1]{c}{\textbf{Cost Model} \\(Excluding Ledger Fees)} &
    No Fees \textbullet\ Creation Fee Only \textbullet\ Usage Fee Only \textbullet\ Creation and Usage Fees \textbullet\ Time-based (Subscription) \textbullet\ Alternative Fee Models \\

    % Technical Transparency
    &
    \SetCell[r=1]{c}{\textbf{Technical Transparency} [OS = Open Source]} &
    Full OS\&No Audit \textbullet\ Partial OS\&No Audit \textbullet\ Closed Source\&No Audit \textbullet\ \textbullet\ Full OS\&Audited \textbullet\ Partial OS\&Audited \textbullet\ Closed Source\&Audited\\

    % GROUP 2: Ledger Specification
    \SetCell[r=3]{c,bg=white}{\rotatebox{90}{\parbox{2.2cm}{\centering \small \textbf{Ledger Specification}}}}
    % Ledger Functionality
    &
    \SetCell[r=1]{c}{\textbf{Ledger Functionality for Identity [MC]}} &
    Credential Anchoring \textbullet\ Credential Storage \textbullet\ Credential Validation \textbullet\ Credential Sharing \textbullet\ Identity Tokenization \textbullet\ Smart Contract Processes \textbullet\ Access Control \textbullet\ On-Chain Evaluation \\
      
    % Consensus Mechanism
    &
    \SetCell[r=1]{c}{\textbf{Consensus Mechanism}} &
    Proof-of-Work \textbullet\ Proof-of-Stake \textbullet\ Proof-of-Authority \textbullet\ Delegated Proof-of-Stake \textbullet\ Byzantine Fault Tolerance \textbullet\ DAG-based \textbullet\ Other  \\
    
    % Ledger Type
    &
    \SetCell[r=1]{c}{\textbf{Ledger Type}} &
    Public Permissionless \textbullet\ Public Permissioned \textbullet\ Private Permissioned  \\
  
    % GROUP 3: Identity and Credential Properties
    \SetCell[r=12]{c,bg=white}{\rotatebox{90}{\parbox{6cm}{\centering \small \textbf{Identity and Credential Properties}}}} 
    % Identity Subject Type
    &
    \SetCell[r=1]{c}{\textbf{Identity Subject Type [MC]}} &
    Human Individuals \textbullet\ Organizations \textbullet\ Devices \textbullet\ Software Applications \textbullet\ Smart Contracts \textbullet\ Digital Assets \textbullet\ Autonomous Agents \textbullet\ Processes/Services  \\
  
    % Identity and Credential Representation
    &
    \SetCell[r=1]{c}{\textbf{Identity and Credential Representation}} &
    Public Key-Based \textbullet\ NFT (transferable) \textbullet\ Soulbound Token \textbullet\ Verifiable Credential \textbullet\ Registry-Based \textbullet\ Anonymous Credential \textbullet\ Digital Identity Certificate  \\
  
    % Credential Issuance Model
    &
    \SetCell[r=1]{c}{\textbf{Credential Issuance Model}} &
    Self-Issued Credentials \textbullet\ Single External Issuer \textbullet\ Multiple Collaborative \textbullet\ Multiple Independent \textbullet\ Hybrid Issuance Model  \\
  
    % Credential Lifespan
    &
    \SetCell[r=1]{c}{\textbf{Credential Lifespan}} &
    Permanent Credentials \textbullet\ Time-Limited Credentials \textbullet\ Activity-Based Credentials \textbullet\ Ephemeral Credentials  \\
  
    % Credential Transferability
    &
    \SetCell[r=1]{c}{\textbf{Credential Transferability}} &
    Full Transferable \textbullet\ Non-Transferable \textbullet\ Conditionally Transferable \textbullet\ Delegable Rights  \\
  
    % Recovery Mechanisms
    &
    \SetCell[r=1]{c}{\textbf{Recovery Mechanisms}} &
    Multi-Signature Recovery \textbullet\ Time-Locked Recovery \textbullet\ Secret Sharing \textbullet\ Escrow-Based Recovery \textbullet\ Biometric Recovery \textbullet\ Other Decentralized Recovery \textbullet\ No Recovery Mechanism \textbullet\ Other Mechanism  \\

  
    % Claim Addition Rights
    &
    \SetCell[r=1]{c}{\textbf{Claim Addition Rights}} &
    Universal Claim Addition \textbullet\ Restricted Claim Addition  \\
  
    % Identifier Type
    &
    \SetCell[r=1]{c}{\textbf{Identifier Type}} &
    Logical Identifiers \textbullet\ Physical Identifiers \textbullet\ DID \textbullet\ Custom  \\
  
    % Initial Claim Provider
    &
    \SetCell[r=1]{c}{\textbf{Initial Claim Provider}} &
    Subject-Provided Claims \textbullet\ Third-Party Claims \textbullet\ Combined Claims  \\
  
    % Privacy Level
    &
    \SetCell[r=1]{c}{\textbf{Privacy Level}} &
    Anonymous Identity \textbullet\ Pseudonymous Identity \textbullet\ Linked Real Identity  \\
  
    % Authentication Mechanism
    &
    \SetCell[r=1]{c}{\textbf{Authentication Mechanism}} &
    Password-Based \textbullet\ Private Key \textbullet\ Hardware Token \textbullet\ Third-Party \textbullet\ Delegated \textbullet\ One-Time Passwords \textbullet\ Biometric \textbullet\ Multi-Factor  \\
  
    % Credential Verifiability
    &
    \SetCell[r=1]{c}{\textbf{Credential Verifiability}} &
    Non-Verifiable Credentials \textbullet\ with Issuer Interaction \textbullet\ without Issuer Interaction \\
  
    % Empty
    
    %\SetCell[r=1]{c}{\textbf{}} &
    %& & \\
    
    
    \end{tblr}
            \caption{Taxonomy dimensions and their characteristics, grouped under "Technical Architecture and Governance", "Ledger Specification", and "Identity and Credential Properties".
        Multiple choice [MC] refers to a dimension not being mutually exclusive.}
        \label{tab:taxonomy-v1-sandro}       
\end{table*}

==> archive/table_taxonomy_v1_old.tex <==
\begin{table}
    \begin{textblock}{12}(2,1.1)  % width in cm, (x,y) coordinates
        \caption{Taxonomy dimensions and their characteristics, grouped under "Technical Architecture and Governance", "Ledger Specification", and "Identity and Credential Properties".\\ 
        Multiple choice [MC] refers to a dimension not being mutually exclusive.}
        \label{tab:taxonomy-v1}
    \end{textblock}
    \vspace{3.4em}
    \begin{tblr}{
        width=\textwidth,
        colspec = {|[1.5pt] X[0.25,c]|[1.5pt]X[1,c]|X[c]|X[c]|X[c]|X[c]|[1.5pt]},
        hlines, vlines,
        rows = {m}, % Middle vertical alignment
        row{1} = {font=\bfseries}, % Bold font for header row
        rowsep = 1.5pt, % Increase the default row separation
        row{1} = {rowsep=4pt}, % Increase the header row height
        % Alternating background colors
        row{2-3} = {bg=gray!10},
        row{4-5} = {},
        row{6-7} = {bg=gray!10},
        row{8-9} = {},
        row{10-11} = {bg=gray!10},
        row{12-13} = {},
        row{14-15} = {bg=gray!10},
        row{16-17} = {},
        row{18-19} = {bg=gray!10},
        row{20-21} = {},
        row{22-23} = {bg=gray!10},
        row{24-25} = {},
        row{26-27} = {bg=gray!10},
        row{28-29} = {},
        row{30-31} = {bg=gray!10},
        row{32-33} = {},
        row{34-35} = {bg=gray!10},
        row{36-37} = {},
        row{38-39} = {bg=gray!10},
        row{40-41} = {},
        row{42-43} = {bg=gray!10},
        row{44-45} = {},
        row{46-47} = {bg=gray!10},
        row{48-49} = {},
        % Horizontal lines adjustments
        hline{1} = {1-6}{1.5pt}, % Top border of table
        hline{2} = {1-6}{1.5pt}, % Under header row
        hline{18} = {1-6}{1.5pt}, % Separation between Group 1 and Group 2
        hline{24} = {1-6}{1.5pt}, % Separation between Group 2 and Group 3
        hline{4,6,8,10,12,14,16,20,22,26,28,30,32,34,36,38,40,42,44,46,48} = {2-6}{0.9pt}, % Lines between dimensions
        hline{50} = {1-6}{1.5pt}, % Bottom horizontal line
    }
    % Header Row
    \SetCell[c=1]{c}\textbf{Group} &
    \SetCell[c=1]{c}\textbf{Dimension} &
    \SetCell[c=4]{c}\textbf{Characteristics} \\

    % GROUP 1: Technical Architecture and Governance
    \SetCell[r=16]{c,bg=white}{\rotatebox{90}{\parbox{6cm}{\centering \small \textbf{Technical Architecture and Governance}}}} &
    % Identity Management Architecture
    \SetCell[r=2]{c}{\textbf{Identity Management Architecture}} &
    Decentralized & Centralized & Federated & Poly-Centric  \\
    & & Self-Sovereign & Siloed & Hybrid & \\
  
    % System Governance Structure
    &
    \SetCell[r=2]{c}{\textbf{System Governance Structure}} &
    Centralized & Consortium & Decentralized & Autonomous \\
    & & Hybrid & & & \\
  
    % Trust Anchor Implementation
    &
    \SetCell[r=2]{c}{\textbf{Trust Anchor Implementation}} &
    Central Authority & Trusted Third Parties & Decentral. Trust Registries & Hardware-Based \\
    & & Decentralized PKI & Web of Trust & & \\
  
    % Identifier Location
    &
    \SetCell[r=2]{c}{\textbf{Identifier Location}} &
    On-Chain Storage & Off-Chain Central. Storage & Off-Chain Decentr. Storage & Local User Storage \\
    & & Hybrid Storage & No Data Stored & & \\
  
    % On-Chain Data Visibility
    &
    \SetCell[r=2]{c}{\textbf{On-Chain Data Visibility}} &
    No On-Chain Data & Hashed Data On-Chain & Encrypted Data On-Chain & Plain Text Data On-Chain \\
    & & & & & \\
  
    % Credential Storage Location
    &
    \SetCell[r=2]{c}{\textbf{Credential Storage Location}} &
    On-Chain & Off-Chain Centralized & Off-Chain Decentralized & Off-Chain at Subject \\
    & & On\&Off-Chain Hybrid & On\&Off-Chain Decentral. & \\
  
    % Cost Model
    &
    \SetCell[r=2]{c}{\textbf{Cost Model} \\(Excluding Ledger Fees)} &
    No Fees & Creation Fee Only & Usage Fee Only & Creation and Usage Fees \\
    & & Time-based (Subscription) & Alternative Fee Models & & \\

    % Technical Transparency
    &
    \SetCell[r=2]{c}{\textbf{Technical Transparency} [OS = Open Source]} &
    Full OS\&No Audit & Partial OS\&No Audit& Closed Source\&No Audit & \\
    & &Full OS\&Audited & Partial OS\&Audited & Closed Source\&Audited\\

    % GROUP 2: Ledger Specification
    \SetCell[r=6]{c,bg=white}{\rotatebox{90}{\parbox{1.5cm}{\centering \small \textbf{Ledger Specification}}}}
    % Ledger Functionality
    &
    \SetCell[r=2]{c}{\textbf{Ledger Functionality for Identity [MC]}} &
    Credential Anchoring & Credential Storage & Credential Validation & Credential Sharing \\
    & Identity Tokenization & & Smart Contract Processes & Access Control & On-Chain Evaluation \\
      
    % Consensus Mechanism
    &
    \SetCell[r=2]{c}{\textbf{Consensus Mechanism}} &
    Proof-of-Work & Proof-of-Stake & Proof-of-Authority & Delegated Proof-of-Stake \\
    & & Byzantine Fault Tolerance & DAG-based & Other & \\
    
    % Ledger Type
    &
    \SetCell[r=2]{c}{\textbf{Ledger Type}} &
    Public Permissionless & Public Permissioned & Private Permissioned & \\
    & & & & & \\
  
    % GROUP 3: Identity and Credential Properties
    \SetCell[r=26]{c,bg=white}{\rotatebox{90}{\parbox{8cm}{\centering \small \textbf{Identity and Credential Properties}}}} 
    % Identity Subject Type
    &
    \SetCell[r=2]{c}{\textbf{Identity Subject Type [MC]}} &
    Human Individuals & Organizations & Devices & Software Applications \\
    & & Smart Contracts & Digital Assets & Autonomous Agents & Processes/Services \\
  
    % Identity and Credential Representation
    &
    \SetCell[r=2]{c}{\textbf{Identity and Credential Representation}} &
    Public Key-Based & NFT (transferable) & Soulbound Token & Verifiable Credential \\
    & & Registry-Based & Anonymous Credential & Digital Identity Certificate & \\
  
    % Credential Issuance Model
    &
    \SetCell[r=2]{c}{\textbf{Credential Issuance Model}} &
    Self-Issued Credentials & Single External Issuer & Multiple Collaborative & Multiple Independent \\
    & & Hybrid Issuance Model & & & \\
  
    % Credential Lifespan
    &
    \SetCell[r=2]{c}{\textbf{Credential Lifespan}} &
    Permanent Credentials & Time-Limited Credentials & Activity-Based Credentials & Ephemeral Credentials \\
    & & & & & \\
  
    % Credential Transferability
    &
    \SetCell[r=2]{c}{\textbf{Credential Transferability}} &
    Full Transferable & Non-Transferable & Conditionally Transferable & Delegable Rights \\
    & & & & & \\
  
    % Recovery Mechanisms
    &
    \SetCell[r=2]{c}{\textbf{Recovery Mechanisms}} &
    Multi-Signature Recovery & Time-Locked Recovery & Secret Sharing & Escrow-Based Recovery \\
    & & Biometric Recovery & Other Decentralized Recovery & No Recovery Mechanism & Other Mechanism \\

  
    % Claim Addition Rights
    &
    \SetCell[r=2]{c}{\textbf{Claim Addition Rights}} &
    Universal Claim Addition & Restricted Claim Addition & & \\
    & & & & & \\
  
    % Identifier Type
    &
    \SetCell[r=2]{c}{\textbf{Identifier Type}} &
    Logical Identifiers & Physical Identifiers & DID & Custom \\
    & & & & & \\
  
    % Initial Claim Provider
    &
    \SetCell[r=2]{c}{\textbf{Initial Claim Provider}} &
    Subject-Provided Claims & Third-Party Claims & Combined Claims & \\
    & & & & & \\
  
    % Privacy Level
    &
    \SetCell[r=2]{c}{\textbf{Privacy Level}} &
    Anonymous Identity & Pseudonymous Identity & Linked Real Identity & \\
    & & & & & \\
  
    % Authentication Mechanism
    &
    \SetCell[r=2]{c}{\textbf{Authentication Mechanism}} &
    Password-Based & Private Key & Hardware Token & Third-Party \\
    & & Delegated & One-Time Passwords & Biometric & Multi-Factor \\
  
    % Credential Verifiability
    &
    \SetCell[r=2]{c}{\textbf{Credential Verifiability}} &
    Non-Verifiable Credentials & with Issuer Interaction & without Issuer Interaction & \\
    & & & & & \\
  
    % Empty
    &
    \SetCell[r=2]{c}{\textbf{}} &
    & & & \\
    & & & & &
    
    \end{tblr}
\end{table}

==> figures/figure_taxonomy-process.tex <==
\begin{figure*}[!t]
    \centering
    \begin{tikzpicture}
        % Main boxes
        \node[draw, rounded corners, minimum width=4cm, minimum height=2cm, align=center] (iter1) at (0,0) {
            Iteration 1: Literature Review\\
            Empirical-to-Conceptual
        };
        
        \node[draw, rounded corners, minimum width=4cm, minimum height=2cm, align=center] (iter2) at (6,0) {
            Iteration 2: Researcher Panel\\
            Empirical-to-Conceptual
        };
        
        \node[draw, rounded corners, minimum width=4cm, minimum height=2cm, align=center] (iter3) at (12,0) {
            Iteration 3: Validation\\
            Conceptual-to-Empirical \&\\
            Empirical-to-Conceptual
        };
        
        % Connect main boxes
        \draw[->, thick] (iter1.east) -- (iter2.west);
        \draw[->, thick] (iter2.east) -- (iter3.west);
        
        % Literature review process
        \node[draw, rounded corners, minimum width=3.5cm, minimum height=1.5cm, align=center] (databases) at (0,-3) {
            5 Databases: IEEE,\\
            Springer, ACM,\\
            Wiley, ScienceDirect
        };
        
        \node[draw, rounded corners, minimum width=3.5cm, minimum height=1.5cm, align=center] (search) at (0,-5.5) {
            "blockchain" OR\\
            "distributed ledger"\\
            AND "identity"
        };
        
        \node[draw, rounded corners, minimum width=3.5cm, minimum height=1.2cm, align=center] (papers) at (0,-8) {
            440 papers → 390\\
            research papers
        };
        
        \node[draw, rounded corners, minimum width=3.5cm, minimum height=0.8cm, align=center] (categories) at (0,-10) {
            11 categories
        };
        
        % Connect literature process
        \draw[->, thick] (iter1.south) -- (databases.north);
        \draw[->, thick] (databases.south) -- (search.north);
        \draw[->, thick] (search.south) -- (papers.north);
        \draw[->, thick] (papers.south) -- (categories.north);
        
        % Researchers
        \node[circle, draw, minimum size=1cm] (r1) at (-1.5,-12) {R1};
        \node[circle, draw, minimum size=1cm] (r2) at (-0.5,-12) {R2};
        \node[circle, draw, minimum size=1cm] (r3) at (0.5,-12) {R3};
        \node[circle, draw, minimum size=1cm] (r4) at (1.5,-12) {R4};
        
        % Connect categories to researchers
        \draw[->, thick] (categories.south) -- +(0,-0.5) -| (r1.north);
        \draw[->, thick] (categories.south) -- +(0,-0.5) -| (r2.north);
        \draw[->, thick] (categories.south) -- +(0,-0.5) -| (r3.north);
        \draw[->, thick] (categories.south) -- +(0,-0.5) -| (r4.north);
        
        % Individual taxonomies
        \node[draw, rounded corners, minimum width=1.2cm, minimum height=0.8cm, align=center] (t1) at (-1.5,-13.5) {Tax 1};
        \node[draw, rounded corners, minimum width=1.2cm, minimum height=0.8cm, align=center] (t2) at (-0.5,-13.5) {Tax 2};
        \node[draw, rounded corners, minimum width=1.2cm, minimum height=0.8cm, align=center] (t3) at (0.5,-13.5) {Tax 3};
        \node[draw, rounded corners, minimum width=1.2cm, minimum height=0.8cm, align=center] (t4) at (1.5,-13.5) {Tax 4};
        
        % Connect researchers to taxonomies
        \draw[->, thick] (r1.south) -- (t1.north);
        \draw[->, thick] (r2.south) -- (t2.north);
        \draw[->, thick] (r3.south) -- (t3.north);
        \draw[->, thick] (r4.south) -- (t4.north);
        
        % Unified taxonomy
        \node[circle, draw, fill=gray!10, minimum size=2cm, align=center] (unified) at (6,-7) {
            Unified\\
            Taxonomy
        };
        
        % Connect taxonomies to unified with better curves
        \draw[->, thick] (t1.east) .. controls +(1,-1) and +(-2,0) .. (unified.west);
        \draw[->, thick] (t2.east) .. controls +(1,-0.5) and +(-1.5,-0.5) .. (unified.west);
        \draw[->, thick] (t3.west) .. controls +(-1,-0.5) and +(-1,-1.5) .. (unified.south west);
        \draw[->, thick] (t4.west) .. controls +(-1,-1) and +(0,-2) .. (unified.south);
        
        % Connect unified to panel
        \draw[->, thick] (unified.north) -- (6,-4) -- (iter2.south);
        
        % Validation sources
        \node[draw, rounded corners, minimum width=3.5cm, minimum height=1.2cm, align=center] (sources) at (12,-3) {
            Surveys, Reviews, \&\\
            Other Taxonomies
        };
        
        % Final taxonomy
        \node[draw, rounded corners, minimum width=3.5cm, minimum height=1.5cm, align=center] (final) at (12,-7) {
            Final Taxonomy\\
            n dimensions, m characteristics
        };
        
        % Connect validation process
        \draw[->, thick, dashed] (iter3.south) -- (sources.north);
        \draw[->, thick] (sources.south) -- (final.north);
        
        % Feedback loop
        \draw[->, thick, dashed] (final.west) to[out=180, in=0] (unified.east);
        
        % Timeline
        \draw[->, ultra thick] (0,-16) -- (6,-16);
        \node at (3,-16.5) {Iterative Development Process};
        
    \end{tikzpicture}
    \caption{Taxonomy Development Process for Blockchain Identity Management}
    \label{fig:taxonomy-development}
\end{figure*}


==> figures/table_ending_conditions.tex <==
% File: ending_conditions_table.tex

\begin{table*}[!htbp]
\caption{Ending Conditions for Taxonomy Development as suggested by Nickerson~et~al.~\cite{nickerson_method_2013}}~.
\centering
\renewcommand{\arraystretch}{0.5} % Adjust row height for better readability
\begin{tabular}{p{0.4cm} p{5cm} p{7cm} p{1.5cm}}
\toprule
\textbf{No.} & \textbf{Condition Keyword} & \textbf{Description} & \textbf{Type} \\
\midrule
O1 & \textbf{All Objects Examined} & All objects or a representative sample have been examined and classified. & Objective \\
O2 & \textbf{No New Dimensions Added} & No new dimensions or characteristics were added in the last iteration. & Objective \\
O3 & \textbf{No Dimensions Merged or Split} & Existing dimensions or characteristics were not merged or split in the last iteration. & Objective \\
O4 & \textbf{Unique Dimensions} & Every dimension is unique and not repeated; there is no duplication of dimensions. & Objective \\
O5 & \textbf{Unique Characteristics in Dimensions} & Every characteristic is unique within its dimension; there is no duplication within a dimension. & Objective \\
O6 & \textbf{Unique Cells (No Duplicates)} & Each cell (combination of characteristics across dimensions) is unique and not repeated. & Objective \\
O7 & \textbf{No Objects Merged or Split} & No objects were merged with similar objects or split into multiple objects in the last iteration. & Objective \\
O8 & \textbf{All Characteristics Used} & At least one object is classified under every characteristic of every dimension; there are no empty characteristics. & Objective \\
\midrule
S1 & \textbf{Conciseness} & The taxonomy is sufficiently simple to be practical; the number of dimensions and characteristics is manageable. & Subjective \\
S2 & \textbf{Robustness} & The taxonomy effectively differentiates between objects; it provides meaningful distinctions. & Subjective \\
S3 & \textbf{Comprehensiveness} & The taxonomy covers all relevant dimensions and characteristics of the domain; it is thorough. & Subjective \\
S4 & \textbf{Extendibility} & The taxonomy can accommodate new objects, dimensions, or characteristics in the future; it is flexible. & Subjective \\
S5 & \textbf{Explanatory Power} & The taxonomy enhances understanding of the domain; it provides insights and explanations. & Subjective \\
\bottomrule
\end{tabular}
\label{tab:ending-conditions}
\end{table*}


==> figures/table_taxonomy-DLT-ID-matrix.tex <==
\begin{table}[ht]
    \centering
    \begin{tabular}{p{1.3em}cc|c}
        & & \multicolumn{2}{c}{\textbf{Identity document location}} \\ 
        & & \multicolumn{2}{c}{} \\
        & & ~~On-chain~~ & Off-chain \\ \cline{3-4} 
        \multirow{2}{*}{\rotatebox{90}{\textbf{Identity usage} 
        \hspace{-2.2em}}}       
        & \rotatebox{90}{Off-chain} & 
        \multicolumn{1}{|c|}{Cell 1} & 
        \multicolumn{1}{c|}{Cell 2} \\ \cline{2-4} 
        & \rotatebox{90}{On-chain  } & 
        \multicolumn{1}{|c|}{Cell 3} & 
        \multicolumn{1}{c|}{Cell 4} \\ \cline{3-4}
    \end{tabular}
    \vspace{0.9em}
    \caption{Classification of different dimensions of distributed ledger-based identity usage and storing.}
    \label{tab:identity}
\end{table}
